Analyzing CLIP's Performance Limitations in Multi-Object Scenarios: A Controlled High-Resolution Study

Contrastive Language-Image Pre-training (CLIP) models have demonstrated remarkable performance in zero-shot classification tasks, yet their efficacy in handling complex multi-object scenarios remains challenging. This study presents a comprehensive analysis of CLIP's performance limitations in multi-object contexts through controlled experiments. We introduce two custom datasets, SimCO and CompCO, to evaluate CLIP's image and text encoders in various multi-object configurations. Our findings reveal significant biases in both encoders: the image encoder favors larger objects, while the text encoder prioritizes objects mentioned first in descriptions. We hypothesize these biases originate from CLIP's training process and provide evidence through analyses of the COCO dataset and CLIP's training progression. Additionally, we extend our investigation to Stable Diffusion models, revealing that biases in the CLIP text encoder significantly impact text-to-image generation tasks. Our experiments demonstrate how these biases affect CLIP's performance in image-caption matching and generation tasks, particularly when manipulating object sizes and their order in captions. This work contributes valuable insights into CLIP's behavior in complex visual environments and highlights areas for improvement in future vision-language models.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/tables/IOC-ComCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Image-based Object Classification On ComCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{ComCo}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{ComCo}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{ComCo}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{ComCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/IOC-SimCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Image-based Object Classification On SimCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/IOR-ComCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Image-based Object Retrieval On ComCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{ComCo}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{ComCo}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{ComCo}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{ComCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/IOR-SimCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Image-based Object Retrieval On SimCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOC-ComCO-Long.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Classification On ComCO dataset in long template}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{ComCo}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{ComCo}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{ComCo}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{ComCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOC-ComCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Classification On ComCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{ComCo}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{ComCo}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{ComCo}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{ComCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOC-SimCO-Long.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Classification On SimCO dataset in long template}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOC-SimCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Classification On SimCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOR-ComCO-Long.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Retrieval On ComCO dataset in long template}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{ComCo}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{ComCo}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{ComCo}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{ComCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOR-ComCO.tex <==
\begin{table*}[ht]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.1}
    \caption{Text-based Object Retrieval On ComCO dataset}
    \label{tab:clip_performance}
    \begin{tabular}{lllcccccc}
    \toprule
    \rowcolor[HTML]{E4E8F2}
    Number of Objects & Dataset & Model & \textbf{Accuracy} & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
    \midrule
    \multirow{16}{*}{n = 2}  & \multirow{8}{*}{SimCO}    
    &  \textit{ViT-H-14 (DFN)}& 92.50 & 66.60 & 33.40 & - & - & - \\
    & & \textit{ViT-SO400M-SigLIP} & 95.93 & 64.46 & 35.54 & - & - & - \\
    & & \textit{ViT-L-14 (datacomp)}& 98.21 & 70.17 & 29.83 & - & - & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 90.68 & 54.39 & 45.61 & - & - & - \\
    & & \textit{ViT-L-14 (laion2b)} & 57.19 & 67.00 & 33.00 & - & - & - \\
    & & \textit{ViT-L-14 (openai)} & 95.97 & 61.93 & 38.07 & - & - & - \\
    & & \textit{ViT-B-32 (openai)} & 96.61 & 56.79 & 43.21 & - & - & - \\
    & & \textit{NegCLIP} & 97.68 & 60.97 & 39.03 & - & - & - \\

    \cmidrule{2-9}
    
    & \multirow{8}{*}{ComCO}    
    &  \textit{ViT-H-14 (DFN)}& 92.50 & 66.60 & 33.40 & - & - & - \\
    & & \textit{ViT-SO400M-SigLIP} & 95.93 & 64.46 & 35.54 & - & - & - \\
    & & \textit{ViT-L-14 (datacomp)}& 98.21 & 70.17 & 29.83 & - & - & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 90.68 & 54.39 & 45.61 & - & - & - \\
    & & \textit{ViT-L-14 (laion2b)} & 57.19 & 67.00 & 33.00 & - & - & - \\
    & & \textit{ViT-L-14 (openai)} & 95.97 & 61.93 & 38.07 & - & - & - \\
    & & \textit{ViT-B-32 (openai)} & 96.61 & 56.79 & 43.21 & - & - & - \\
    & & \textit{NegCLIP} & 97.68 & 60.97 & 39.03 & - & - & - \\
    
    \midrule 
    \multirow{16}{*}{n = 3} & \multirow{8}{*}{SimCO}   
    &  \textit{ViT-H-14 (DFN)}& 84.29 & 63.79 & 22.86 & 13.35 & - & - \\
    & & \textit{ViT-SO400M-SigLIP} & 85.47 & 55.86 & 23.70 & 20.45 & - & - \\
    & & \textit{ViT-L-14 (datacomp)}& 84.84 & 71.95 & 17.82 & 10.23 & - & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 60.37 & 39.22 & 30.07 & 30.71 & - & - \\
    & & \textit{ViT-L-14 (laion2b)} & 32.67 & 66.03 & 20.99 & 12.98 & - & - \\
    & & \textit{ViT-L-14 (openai)} & 79.13 & 55.75 & 25.20 & 19.06 & - & - \\
    & & \textit{ViT-B-32 (openai)} & 79.53 & 52.16 & 27.14 & 20.70 & - & - \\
    & & \textit{NegCLIP} & 80.28 & 56.94 & 27.65 & 15.41 & - & - \\

    \cmidrule{2-9}
    & \multirow{8}{*}{ComCO}    
    &  \textit{ViT-H-14 (DFN)}& 84.29 & 63.79 & 22.86 & 13.35 & - & - \\
    & & \textit{ViT-SO400M-SigLIP} & 85.47 & 55.86 & 23.70 & 20.45 & - & - \\
    & & \textit{ViT-L-14 (datacomp)}& 84.84 & 71.95 & 17.82 & 10.23 & - & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 60.37 & 39.22 & 30.07 & 30.71 & - & - \\
    & & \textit{ViT-L-14 (laion2b)} & 32.67 & 66.03 & 20.99 & 12.98 & - & - \\
    & & \textit{ViT-L-14 (openai)} & 79.13 & 55.75 & 25.20 & 19.06 & - & - \\
    & & \textit{ViT-B-32 (openai)} & 79.53 & 52.16 & 27.14 & 20.70 & - & - \\
    & & \textit{NegCLIP} & 80.28 & 56.94 & 27.65 & 15.41 & - & - \\
     
    \midrule
    \multirow{16}{*}{n = 4} & \multirow{8}{*}{SimCO}   
    
    &  \textit{ViT-H-14 (DFN)}& 63.50 & 60.82 & 20.12 & 11.68 & 7.38 & - \\
    & & \textit{ViT-SO400M-SigLIP} & 64.50 & 52.46 & 20.09 & 13.14 & 14.31 & - \\
    & & \textit{ViT-L-14 (datacomp)}& 61.18 & 72.23 & 14.62 & 8.27 & 4.88 & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 31.43 & 30.43 & 25.65 & 22.63 & 21.29 & - \\
    & & \textit{ViT-L-14 (laion2b)} & 15.60 & 61.85 & 20.65 & 10.69 & 6.80 & - \\
    & & \textit{ViT-L-14 (openai)} & 49.73 & 48.59 & 23.60 & 16.00 & 11.81 & - \\
    & & \textit{ViT-B-32 (openai)} & 51.75 & 48.62 & 26.35 & 15.50 & 9.53 & - \\
    & & \textit{NegCLIP} & 52.52 & 53.43 & 26.58 & 14.22 & 5.77 & - \\

    \cmidrule{2-9}
    & \multirow{8}{*}{ComCO}    
    &  \textit{ViT-H-14 (DFN)}& 63.50 & 60.82 & 20.12 & 11.68 & 7.38 & - \\
    & & \textit{ViT-SO400M-SigLIP} & 64.50 & 52.46 & 20.09 & 13.14 & 14.31 & - \\
    & & \textit{ViT-L-14 (datacomp)}& 61.18 & 72.23 & 14.62 & 8.27 & 4.88 & - \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 31.43 & 30.43 & 25.65 & 22.63 & 21.29 & - \\
    & & \textit{ViT-L-14 (laion2b)} & 15.60 & 61.85 & 20.65 & 10.69 & 6.80 & - \\
    & & \textit{ViT-L-14 (openai)} & 49.73 & 48.59 & 23.60 & 16.00 & 11.81 & - \\
    & & \textit{ViT-B-32 (openai)} & 51.75 & 48.62 & 26.35 & 15.50 & 9.53 & - \\
    & & \textit{NegCLIP} & 52.52 & 53.43 & 26.58 & 14.22 & 5.77 & - \\
     
    \midrule
    \multirow{16}{*}{n = 5}& \multirow{8}{*}{SimCO}   
    
    
    &  \textit{ViT-H-14 (DFN)}& 38.58 & 56.81 & 18.69 & 12.20 & 7.22 & 5.09 \\
    & & \textit{ViT-SO400M-SigLIP} & 39.80 & 50.00 & 17.61 & 10.74 & 9.26 & 12.38 \\
    & & \textit{ViT-L-14 (datacomp)}& 37.09 & 71.04 & 13.18 & 8.09 & 4.56 & 3.13 \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 11.09 & 24.57 & 21.35 & 19.94 & 18.57 & 15.58 \\
    & & \textit{ViT-L-14 (laion2b)} & 6.86 & 57.66 & 20.05 & 11.73 & 5.73 & 4.84 \\
    & & \textit{ViT-L-14 (openai)} & 21.50 & 40.77 & 22.48 & 15.81 & 11.51 & 9.43 \\
    & & \textit{ViT-B-32 (openai)} & 25.05 & 43.86 & 26.41 & 15.44 & 8.57 & 5.72 \\
    & & \textit{NegCLIP} & 27.53 & 49.82 & 25.03 & 15.36 & 7.02 & 2.77 \\


    \cmidrule{2-9}
    & \multirow{8}{*}{ComCO}    
    &  \textit{ViT-H-14 (DFN)}& 38.58 & 56.81 & 18.69 & 12.20 & 7.22 & 5.09 \\
    & & \textit{ViT-SO400M-SigLIP} & 39.80 & 50.00 & 17.61 & 10.74 & 9.26 & 12.38 \\
    & & \textit{ViT-L-14 (datacomp)}& 37.09 & 71.04 & 13.18 & 8.09 & 4.56 & 3.13 \\
    & & \textit{xlm-roberta-large-ViT-H-14}& 11.09 & 24.57 & 21.35 & 19.94 & 18.57 & 15.58 \\
    & & \textit{ViT-L-14 (laion2b)} & 6.86 & 57.66 & 20.05 & 11.73 & 5.73 & 4.84 \\
    & & \textit{ViT-L-14 (openai)} & 21.50 & 40.77 & 22.48 & 15.81 & 11.51 & 9.43 \\
    & & \textit{ViT-B-32 (openai)} & 25.05 & 43.86 & 26.41 & 15.44 & 8.57 & 5.72 \\
    & & \textit{NegCLIP} & 27.53 & 49.82 & 25.03 & 15.36 & 7.02 & 2.77 \\
    
    
    \bottomrule
    \end{tabular}
    \end{table*}

==> sec/tables/TOR-SimCO-Long.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Retrieval On SimCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/TOR-SimCO.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.2}
\caption{Text-based Object Retrieval On ComCO dataset}
\label{tab:clip_performance}
\begin{tabular}{llcccccc}
\toprule
\rowcolor[HTML]{E4E8F2}
Number of Objects & Dataset & Model & \textbf{First Object} & \textbf{Second Object} & \textbf{Third Object} & \textbf{Fourth Object} & \textbf{Fifth Object} \\ 
\midrule
\multirow{11}{*}{n = 2} & \multirow{11}{*}{SimCO}   
& \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
& & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
& & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
& & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
& & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\

\midrule
\multirow{11}{*}{n = 3} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 4} & \multirow{11}{*}{SimCO}   


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 
\midrule
\multirow{11}{*}{n = 5} & \multirow{11}{*}{SimCO}  


 & \textit{ViT-H-14 (DFN)} & - & - & - & - & - \\
 & & \textit{ViT-SO400M-SigLIP} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (datacomp)} & - & - & - & - & - \\
 & & \textit{xlm-roberta-large-ViT-H-14} & - & - & - & - & - \\
 & & \textit{ViT-L-14 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-L-14 (openai)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (datacomp)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (laion2b)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (metaclip)} & - & - & - & - & - \\
& & \textit{ViT-B-32 (openai)} & - & - & - & - & - \\
& & \textit{NegCLIP} & - & - & - & - & - \\
 


\bottomrule
\end{tabular}
\end{table*}

==> sec/tables/domainnet-table.tex <==
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\caption{Performance of various CLIP models on different datasets}
\label{tab:clip_performance}
\begin{tabular}{lllllllllllllllllllll}
\toprule
\rowcolor[HTML]{E4E8F2}
\#objects & Scenario     & Model                        & Accuracy & Word1 & Word2 & Word3 & Word4 & Word5 & F1 Score & mAP   & P@1 & R@1 & P@2 & R@2 & P@3 & R@3 & P@4 & R@4 & P@5 & R@5 \\
\multirow{16}{*}{2}
  & \multirow{8}{*}{Large\_Small} 
  & ViT-H-14 dfn5b    & 83.13 & 68.77 & 31.23 & - & - & - & 90.56 & 85.99 & 81.50 & 40.75 & 90.56 & 90.56 & - & - & - & - & - & - \\
  &  & ViT-14-SigLIP  & 93.35 & 69.29 & 30.71 & - & - & - & 95.43 & 93.14 & 90.86 & 45.43 & 95.43 & 95.43 & - & - & - & - & - & - \\
  &  & ViT-L-14 datacomp     & 98.86 & 70.51 & 29.49 & - & - & - & 98.73 & 98.09 & 97.46 & 48.73 & 98.73 & 98.73 & - & - & - & - & - & - \\
  &  & xlm-roberta-ViT-H-14  & 89.02 & 61.73 & 38.27 & - & - & - & 94.27 & 91.89 & 90.16 & 45.08 & 94.27 & 94.27 & - & - & - & - & - & - \\
  &  & ViT-L-14 laion2b  & 56.46 & 74.33 & 25.67 & - & - & - & 75.72 & 65.90 & 57.65 & 28.83 & 75.72 & 75.72 & - & - & - & - & - & - \\
  &  & ViT-L-14 openai   & 96.43 & 66.74 & 33.26 & - & - & - & 97.62 & 96.43 & 95.24 & 47.62 & 97.62 & 97.62 & - & - & - & - & - & - \\
  &  & ViT-B-32 openai   & 96.70 & 70.64 & 29.36 & - & - & - & 97.62 & 96.43 & 95.24 & 47.62 & 97.62 & 97.62 & - & - & - & - & - & - \\
  &  & NegCLIP    & 97.51 & 72.88 & 27.12 & - & - & - & 97.49 & 96.23 & 94.97 & 47.49 & 97.49 & 97.49 & - & - & - & - & - & - \\
\cmidrule{2-21}
  & \multirow{8}{*}{Small\_Large} 
      & ViT-H-14-dfn5b    & 82.80 & 63.49 & 36.51 & - & - & - & 91.10 & 86.75 & 82.42 & 41.21 & 91.10 & 91.10 & - & - & - & - & - & - \\
      &  & ViT-L-14-SigLIP  & 94.16 & 49.57 & 50.43 & - & - & - & 96.38 & 94.58 & 92.81 & 46.40 & 96.38 & 96.38 & - & - & - & - & - & - \\
      &  & ViT-L-14 datacomp& 98.81 & 66.45 & 33.55 & - & - & - & 99.19 & 98.78 & 98.38 & 49.19 & 99.19 & 99.19 & - & - & - & - & - & - \\
      &  & xlm-roberta-ViT-H-14 & 90.27 & 53.86 & 46.14 & - & - & - & 95.08 & 92.74 & 90.59 & 45.29 & 95.08 & 95.08 & - & - & - & - & - & - \\
      &  & ViT-L-14 laion2b & 60.14 & 42.27 & 57.73 & - & - & - & 78.04 & 68.86 & 60.52 & 30.26 & 78.04 & 78.04 & - & - & - & - & - & - \\
      &  & ViT-L-14 openai   & 97.13 & 65.81 & 34.19 & - & - & - & 98.35 & 97.53 & 96.70 & 48.35 & 98.35 & 98.35 & - & - & - & - & - & - \\
      &  & ViT-B-32 openai   & 97.30 & 57.92 & 42.08 & - & - & - & 98.16 & 97.24 & 96.32 & 48.16 & 98.16 & 98.16 & - & - & - & - & - & - \\
      &  & NegCLIP    & 98.65 & 65.52 & 34.48 & - & - & - & 98.81 & 98.22 & 97.62 & 48.81 & 98.81 & 98.81 & - & - & - & - & - & - \\
\cmidrule{1-21}
\multirow{16}{*}{3}
  & \multirow{8}{*}{Large\_Small} 
        & ViT-H-14 dfn5b    & 69.17 & 67.47 & 24.94 & 7.58 & - & - & 87.80 & 78.43 & 67.50 & 22.50 & 81.69 & 54.46 & 87.80 & 87.80 & - & - & - & - \\
        &  & ViT-14-SigLIP  & 69.50 & 71.05 & 3.04 & 25.91 & - & - & 88.16 & 80.35 & 75.18 & 25.06 & 82.53 & 55.02 & 88.16 & 88.16 & - & - & - & - \\
        &  & ViT-L-14 datacomp      & 84.37 & 74.55 & 17.56 & 7.88 & - & - & 93.24 & 88.15 & 82.96 & 27.65 & 89.86 & 59.91 & 93.24 & 93.24 & - & - & - & - \\
        &  & xlm-roberta-ViT-H-14  & 62.03 & 48.56 & 33.13 & 18.31 & - & - & 86.62 & 76.92 & 66.25 & 22.08 & 80.64 & 53.76 & 86.62 & 86.62 & - & - & - & - \\
        &  & ViT-L-14 laion2b  & 34.18 & 85.28 & 4.43 & 10.28 & - & - & 73.57 & 57.73 & 44.46 & 14.82 & 62.93 & 41.95 & 73.57 & 73.57 & - & - & - & - \\
        &  & ViT-L-14 openai   & 75.28 & 62.50 & 24.86 & 12.64 & - & - & 90.79 & 83.82 & 73.82 & 24.61 & 86.24 & 57.49 & 90.79 & 90.79 & - & - & - & - \\
        &  & ViT-B-32 openai   & 68.04 & 64.86 & 27.74 & 7.39 & - & - & 87.99 & 79.73 & 64.31 & 21.44 & 81.99 & 54.66 & 87.99 & 87.99 & - & - & - & - \\
        &  & NegCLIP    & 67.28 & 69.21 & 27.73 & 3.05 & - & - & 87.51 & 77.39 & 62.68 & 20.89 & 81.26 & 54.17 & 87.51 & 87.51 & - & - & - & - \\
  \cmidrule{2-21}
  & \multirow{8}{*}{Small\_Large} 
          & ViT-H-14 dfn5b    & 79.18 & 49.66 & 24.39 & 25.96 & - & - & 92.68 & 86.74 & 78.69 & 26.23 & 89.02 & 59.35 & 92.68 & 92.68 & - & - & - & - \\
          &  & ViT-14-SigLIP  & 74.91 & 50.76 & 1.88 & 47.36 & - & - & 90.54 & 83.66 & 77.45 & 25.82 & 85.83 & 57.22 & 90.54 & 90.54 & - & - & - & - \\
          &  & ViT-L-14 datacomp    & 93.40 & 61.32 & 10.19 & 28.49 & - & - & 97.06 & 94.77 & 92.10 & 30.70 & 95.59 & 63.73 & 97.06 & 97.06 & - & - & - & - \\
          &  & xlm-roberta-ViT-H-14  & 70.42 & 29.95 & 28.88 & 41.17 & - & - & 89.90 & 82.23 & 73.45 & 24.48 & 85.05 & 56.70 & 89.90 & 89.90 & - & - & - & - \\
          &  & ViT-L-14 laion2b  & 51.05 & 45.76 & 5.08 & 49.15 & - & - & 81.14 & 68.45 & 55.16 & 18.39 & 72.26 & 48.17 & 81.14 & 81.14 & - & - & - & - \\
          &  & ViT-L-14 openai   & 83.78 & 60.56 & 18.98 & 20.46 & - & - & 94.27 & 87.56 & 83.45 & 27.82 & 91.40 & 60.93 & 94.27 & 94.27 & - & - & - & - \\
          &  & ViT-B-32 openai   & 85.88 & 51.95 & 19.14 & 28.90 & - & - & 94.88 & 86.45 & 85.45 & 28.48 & 92.32 & 61.55 & 94.88 & 94.88 & - & - & - & - \\
          &  & NegCLIP    & 85.88 & 59.57 & 27.77 & 12.66 & - & - & 95.22 & 88.12 & 85.78 & 28.59 & 92.83 & 61.89 & 95.22 & 95.22 & - & - & - & - \\
  \cmidrule{1-21}

          \multirow{16}{*}{4}
            & \multirow{8}{*}{Large\_Small} 
            & ViT-H-14 dfn5bb    & 54.03 & 62.76 & 21.62 & 8.21 & 7.41 & - & 86.86 & 74.48 & 58.84 & 14.71 & 75.26 & 37.63 & 82.50 & 61.87 & 86.86 & 86.86 & - & - \\
            &  & ViT-14-SigLIP  & 65.33 & 47.19 & 22.43 & 15.23 & 15.15 & - & 90.21 & 80.65 & 67.50 & 16.87 & 80.80 & 40.40 & 86.95 & 65.21 & 90.21 & 90.21 & - & - \\
            &  & ViT-L-14 datacomp     & 51.65 & 61.36 & 24.29 & 13.09 & 1.26 & - & 86.75 & 73.45 & 53.98 & 13.49 & 74.58 & 37.29 & 82.35 & 61.76 & 86.75 & 86.75 & - & - \\
            &  & xlm-roberta-ViT-H-14  & 36.40 & 41.31 & 32.24 & 21.69 & 4.75 & - & 83.15 & 67.85 & 49.32 & 12.33 & 68.52 & 34.26 & 78.02 & 58.52 & 83.15 & 83.15 & - & - \\
            &  & ViT-L-14 laion2b  & 30.99 & 67.36 & 18.50 & 12.22 & 1.92 & - & 79.58 & 61.90 & 39.26 & 9.82 & 63.17 & 31.58 & 73.32 & 54.99 & 79.58 & 79.58 & - & - \\
            &  & ViT-L-14 openai   & 47.49 & 60.36 & 25.40 & 3.87 & 10.36 & - & 86.07 & 72.44 & 54.14 & 13.53 & 72.66 & 36.33 & 81.45 & 61.09 & 86.07 & 86.07 & - & - \\
            &  & ViT-B-32 openai   & 38.67 & 70.07 & 22.52 & 4.90 & 2.52 & - & 82.42 & 66.04 & 43.92 & 10.98 & 65.71 & 32.86 & 76.62 & 57.46 & 82.42 & 82.42 & - & - \\
            &  & NegCLIP    & 32.23 & 47.99 & 35.74 & 16.28 & 0.00 & - & 81.77 & 63.32 & 35.32 & 8.83 & 63.68 & 31.84 & 75.70 & 56.77 & 81.77 & 81.77 & - & - \\

  \cmidrule{2-21}
   & \multirow{8}{*}{Small\_Large} 
              & ViT-H-14 dfn5bb     & 64.09 & 45.65 & 21.27 & 13.16 & 19.92 & - & 90.64 & 81.18 & 66.79 & 16.70 & 81.67 & 40.83 & 87.52 & 65.64 & 90.64 & 90.64 & - & - \\
              &  & ViT-14-SigLIP  & 74.20 & 32.43 & 23.10 & 17.86 & 26.60 & - & 93.09 & 86.14 & 76.10 & 19.02 & 86.32 & 43.16 & 90.79 & 68.09 & 93.09 & 93.09 & - & - \\
              &  & ViT-L-14 datacomp    & 84.10 & 44.76 & 23.15 & 16.72 & 15.37 & - & 95.73 & 91.28 & 84.32 & 21.08 & 91.48 & 45.74 & 94.30 & 70.73 & 95.73 & 95.73 & - & - \\
              &  & xlm-roberta-ViT-H-14  & 47.54 & 25.48 & 27.87 & 21.39 & 25.26 & - & 86.38 & 73.16 & 54.84 & 13.71 & 73.45 & 36.72 & 81.99 & 61.49 & 86.38 & 86.38 & - & - \\
              &  & ViT-L-14 laion2b  & 51.54 & 26.44 & 30.33 & 23.29 & 19.94 & - & 86.36 & 73.64 & 56.25 & 14.06 & 73.20 & 36.60 & 81.81 & 61.36 & 86.36 & 86.36 & - & - \\
              &  & ViT-L-14 openai   & 56.03 & 63.51 & 14.09 & 8.88 & 13.51 & - & 88.55 & 76.98 & 63.06 & 15.77 & 77.42 & 38.71 & 84.73 & 63.55 & 88.55 & 88.55 & - & - \\
              &  & ViT-B-32 openai   & 61.55 & 55.98 & 22.76 & 8.17 & 13.09 & - & 89.71 & 79.84 & 65.66 & 16.41 & 79.83 & 39.91 & 86.32 & 64.74 & 89.71 & 89.71 & - & - \\
              &  & NegCLIP    & 59.92 & 35.29 & 39.35 & 20.13 & 5.23 & - & 89.86 & 79.37 & 61.93 & 15.48 & 79.75 & 39.87 & 86.48 & 64.86 & 89.86 & 89.86 & - & - \\
  \cmidrule{1-21}

\multirow{16}{*}{5}
                & \multirow{8}{*}{Large\_Small} 
                & ViT-H-14 dfn5b   & 37.37 & 63.39 & 13.60 & 6.51 & 7.38 & 9.12 & 85.46 & 74.35 & 53.70 & 10.74 & 69.12 & 27.65 & 77.77 & 46.66 & 81.84 & 65.47 & 85.46 & 85.46 \\
                &  & ViT-14-SigLIP  & 30.83 & 43.68 & 20.70 & 8.95 & 9.82 & 16.84 & 83.24 & 73.32 & 50.14 & 10.03 & 63.93 & 25.57 & 73.12 & 43.87 & 79.06 & 63.24 & 83.24 & 83.24 \\
                &  & ViT-L-14 datacomp     & 12.11 & 75.00 & 8.93 & 8.04 & 7.14 & 0.89 & 77.07 & 67.29 & 45.48 & 9.10 & 49.92 & 19.97 & 64.72 & 38.83 & 71.34 & 57.07 & 77.07 & 77.07 \\
                &  & xlm-roberta-ViT-H-14  & 2.60 & 12.50 & 22.92 & 14.58 & 29.17 & 20.83 & 70.63 & 56.32 & 34.13 & 6.83 & 40.62 & 16.25 & 54.52 & 32.71 & 63.97 & 51.17 & 70.63 & 70.63 \\
                &  & ViT-L-14 laion2b   & 18.98 & 68.66 & 12.54 & 6.27 & 10.83 & 1.71 & 78.43 & 65.48 & 43.37 & 8.67 & 57.27 & 22.91 & 67.86 & 40.71 & 73.50 & 58.80 & 78.43 & 78.43 \\
                &  & ViT-L-14 openai   & 2.22 & 80.49 & 2.44 & 4.88 & 2.44 & 9.76 & 66.04 & 56.43 & 33.21 & 6.64 & 37.99 & 15.20 & 46.67 & 28.00 & 57.60 & 46.08 & 66.04 & 66.04 \\
                &  & ViT-B-32 openai   & 1.24 & 78.26 & 8.70 & 4.35 & 0.00 & 8.70 & 60.63 & 52.23 & 23.20 & 4.64 & 29.94 & 11.97 & 38.94 & 23.36 & 50.87 & 40.69 & 60.63 & 60.63 \\
                &  & NegCLIP    & 3.03 & 73.21 & 5.36 & 10.71 & 7.14 & 3.57 & 67.77 & 56.40 & 32.13 & 6.43 & 37.13 & 14.85 & 49.25 & 29.55 & 59.73 & 47.79 & 67.77 & 67.77 \\
  \cmidrule{2-21}
                  & \multirow{8}{*}{Small\_Large} 
                  & ViT-H-14 dfn5b    & 45.05 & 48.62 & 9.96 & 6.48 & 8.88 & 26.05 & 87.44 & 77.26 & 55.16 & 11.03 & 71.96 & 28.78 & 80.04 & 48.03 & 84.30 & 67.44 & 87.44 & 87.44 \\
                  &  & ViT-14-SigLIP  & 36.78 & 32.50 & 23.53 & 12.79 & 10.15 & 21.03 & 85.37 & 75.67 & 54.57 & 10.91 & 67.71 & 27.08 & 75.97 & 45.58 & 81.72 & 65.38 & 85.37 & 85.37 \\
                  &  & ViT-L-14 datacomp     & 26.99 & 64.53 & 8.62 & 6.21 & 5.41 & 15.23 & 83.29 & 73.34 & 44.35 & 8.87 & 61.57 & 24.63 & 72.49 & 43.49 & 79.11 & 63.29 & 83.29 & 83.29 \\
                  &  & xlm-roberta-ViT-H-14  & 2.16 & 12.50 & 2.50 & 15.00 & 15.00 & 55.00 & 74.16 & 62.72 & 36.34 & 7.27 & 45.08 & 18.03 & 58.16 & 34.89 & 67.86 & 54.29 & 74.16 & 74.16 \\
                  &  & ViT-L-14 laion2b  & 37.26 & 36.14 & 18.14 & 9.14 & 11.90 & 24.67 & 84.40 & 72.83 & 53.06 & 10.61 & 66.14 & 26.46 & 74.89 & 44.93 & 80.50 & 64.40 & 84.40 & 84.40 \\
                  &  & ViT-L-14 openai   & 1.95 & 75.00 & 2.78 & 0.00 & 5.56 & 16.67 & 66.48 & 55.64 & 31.04 & 6.21 & 36.05 & 14.42 & 46.78 & 28.07 & 58.18 & 46.54 & 66.48 & 66.48 \\
                  &  & ViT-B-32 openai   & 2.97 & 70.91 & 14.55 & 3.64 & 3.64 & 5.45 & 64.37 & 54.57 & 23.42 & 4.68 & 30.56 & 12.22 & 43.25 & 25.95 & 55.49 & 44.39 & 64.37 & 64.37 \\
                  &  & NegCLIP    & 5.52 & 74.51 & 7.84 & 8.82 & 3.92 & 4.90 & 74.03 & 62.94 & 35.26 & 7.05 & 43.48 & 17.39 & 57.35 & 34.41 & 67.54 & 54.03 & 74.03 & 74.03 \\
\bottomrule
\end{tabular}
\end{table*}

